Explicit multiplicities in the cuspidal spectrum of SU(n,1)

This paper investigates the cuspidal spectrum of the quotient of the real Lie group $G= SU(n,1)$ and a principal congruence subgroup $\Gamma(m)$ for $m\geq 3$, focusing on the multiplicities of integrable discrete series representations. Using the Selberg trace formula, we derive an explicit formula for the multiplicity $m(\Gamma(m), \pi_\tau)$ of a representation $\pi_\tau$ of integrable discrete series of $G$ within $L^2(\Gamma(m) \backslash G)$. The formula involves the Harish-Chandra parameter $\tau$, the discriminant $D_\ell$ of the imaginary quadratic field $\ell$ over which $G$ is defined and special values of the Dirichlet $L$-function $L_\ell$ associated to $\ell$. We apply these results on the one hand to compute the cuspidal cohomology of locally symmetric spaces $\Gamma(m) \backslash G / K$, where $K$ is a maximal compact subgroup of $G$. On the other hand we use them to reprove a known rationality result involving the values of $L_\ell$ at odd positive integers and make them more explicit. This work extends previous studies on real and quaternionic hyperbolic spaces to the complex hyperbolic case, contributing to the understanding of the spectrum of $\mathbb{R}$-rank one algebraic groups.

==> 3Volume.tex <==


\section{Prasad's Volume Formula} \label{prasad}
We would like to apply Prasad's Volume Formula (\cite{prasad}, Theorem 3.7) to $\mathrm{G}=\su(n,1)$ with $S=\{\infty\}$ to compute $\mathrm{vol}(\Gamma \backslash G)$. To do this, we will define a principal arithmetic group $\Gamma$ explicitly below. We will then look at subgroups $\Gamma(m)$ of $\Gamma$ of finite index $h_m$. We have
$$
\mathrm{vol}(\Gamma(m) \backslash G) = h_m\cdot  \mathrm{vol}(\Gamma \backslash G),
$$
so it suffices to compute $\mathrm{vol}(\Gamma\backslash G)$. 



\subsection{The arithmetic subgroup} \label{arithmetic-subgroup}
We interpret $\mathrm{G}_{\Z}$ as the integer points of the $\Q$-algebraic group $\mathrm{G}=\mathrm{SU}(n,1)$ corresponding to the quadratic extension $\ell=\Q(\sqrt{-k})$ of $\Q$. $\mathrm{G}_{\Z}$ is a lattice in $G$. We call an arithmetic subgroup of $G$ an \textit{arithmetic lattice}, if it is commensurable with $\mathrm{G}_{\Z}$ \cite[§2]{emery}. 
\begin{cor}
    If $n$ is even, the commensurability class of nonuniform arithmetic lattices $\Gamma$ of $G$ is unique. If $n$ is odd, commensurability classes of $G$ are in one-to-one correspondence with $\Q^\times / N_{\ell/\Q}(\ell^\times)$.
\end{cor}
Let $(\mathrm{K}_p)_p$ be a coherent collection of parahoric subgroups of $\mathrm{G}(\Q_p)$. As in \cite[§3.4]{prasad} or \cite[§2.2 ]{emery}, an arithmetic subgroup $\Gamma$ of $G$ can be constructed: 
By strong approximation, 
$$
G \cdot \prod_{p\ prime} \mathrm{K}_p \cdot \mathrm{G}(\Q)=\mathrm{G}(\mathbb{A}).
$$
\begin{de} \label{defgamma}
    We say that an arithmetic subgroup $\Gamma$ of $G$ is a \textit{principal arithmetic lattice} if it is the image of 
    $$
    \mathrm{G}(\Q)\cap \left(G\cdot \prod_{p\ prime} \mathrm{K}_p \right)
    $$
    under the natural projection
    $$
     G \cdot \prod_{p\ prime} \mathrm{K}_p \rightarrow G,
    $$
    where $\mathrm{G}(\Q)$ is understood as embedded diagonally into $\mathrm{G}(\mathbb{A})$ and $(\mathrm{K}_p)_p$ is a coherent collection of parahoric subgroups of $\mathrm{G}(\Q_p)$.
\end{de}
We denote by $T_\ell$ the set of finite places $p$ where the the local group $\mathrm{G}(\Q_p)$ is not quasi-split.
Let $(\mathrm{K}_p)_p$
be a coherent collection of parahoric subgroups $\mathrm{K}_p$ of $\mathrm{G}(\Q_p)$ of maximal volume. This ensures that $\mathrm{K}_p$ is special for all $p$ and if $p\not \in T_\ell$ is not ramified in $\ell$, then $\mathrm{K}_p$ is hyperspecial (\cite[Section 3.1]{emery}). The covolume of the principal arithmetic lattice $\Gamma$ is now independet of the choice of the individual $\mathrm{K}_p$.
We denote the quasi split unitary group, such that $\mathrm{G}$ is an inner form of it by $\mathscr{G}$. We noted above, that $\mathscr{G}=\mathrm{SU}(\frac{n+1}{2},\frac{n+1}{2})$ if $n$ is odd and $\mathscr{G}=\mathrm{SU}(\frac{n}{2}+1,\frac{n}{2})$ if $n$ is even. As described in \cite[2.2]{prasad}, we let $\mathrm{G}_p$ be the smooth affine $\Z_p$-group scheme associated with the parahoric subgroup $\mathrm{K}_p$ of $\mathrm{G}(\Q_p).$ Analogously, we let $\mathscr{G}_p$ be the canonical smooth affine $\Z_p$-group scheme of $\mathscr{G}(\Q_p)$ associated by Bruhat-Tits theory \cite[Section 4]{gr} and let $\mathscr{K}_p$ be the corresponding parahoric subgroup.
Furthermore, we denote by $\overline{\mathrm{G}}_p$ and $\overline{\mathscr{G}}_p$ the the reduction modulo $p$ of $\mathrm{G}_p$ and $\mathscr{G}_p$ over the residue field $\mathbb{F}_p$. Both are connected and admit a Levi decomposition
$$
\overline{\mathrm{G}_p} = \overline{\mathrm{M}_p} \cdot \mathrm{R}_u(\overline{\mathrm{G}_p})
$$
and 
$$
\overline{\mathscr{G}_p} = \overline{\mathscr{M}_p} \cdot \mathrm{R}_u(\overline{\mathscr{G}_p}),
$$
where $\mathrm{R}_u$ denotes the unipotent radical. Computing the corresponding integral models, we can determine the groups $\overline{M}_p$ and $\overline{\mathscr{M}}_p$. This is necessary for Prasad's Volume formula (\cite{prasad}):
\begin{align} \label{pra}
    \mu_{EP}(\Gamma\backslash G)=\chi(\C \mathbb{P}^n) D_\ell^{s(n)} \left( \prod_{r=1}^n \frac{r!}{(2\pi)^{r+1}}\right) \cdot \prod_p \frac{p^{\frac{1}{2}(\dim(\overline{M}_p) + \dim(\overline{\mathscr{M}}_p))}}{|\overline{M}_p(\mathbb{F}_{p})|},
\end{align}
where 
\begin{align*}
    s(n)\coloneqq \left \{ 
    \begin{matrix}
        \frac{(n-1)(n+2)}{4} & \ if\ n\ is\ odd, \\
        \frac{n(n+3)}{4} & \ if\ n\ is\ even.
    \end{matrix}
    \right.
\end{align*}
Therefore, we study special unitary groups over local fields. We will define the parahoric subgroups, the integral models and compute the reductive quotient over the special fibres in every case. 





 
\subsection{Hermitian spaces over local fields}
Let $L/\Q_p$ be an imaginary quadratic field extension. Now for $q\in \N$ we set $V\coloneqq L^q$ and we look at hermitian forms $h$ on $V$ given by (with a chosen basis)
$$
h(\mathbf{x},\mathbf{y})\coloneqq \mathbf{y}^\dagger S_h \mathbf{x}
$$
where $\overline{\cdot}$ denotes the non-trivial element in the Galois group of $L/\Q$ and $S_h$ is a hermitian matrix with respect to $\overline{\cdot}$. We define the following (\cite[Section 3]{hanke}):
\begin{itemize}
    \item $H\coloneqq L^2$ is the split rank-two hermitian space over $L$ with hermitian form $h$ given by 
    $$
    S_h=\left(\begin{matrix}
0 & 1  \\
1 & 0  \\
\end{matrix}\right).
    $$
    \item Let $A_{L}$ be the ring of integers of $L$. 
    \item We denote by $\mathscr{D}$ the different of $L/\Q_p$.
    \item Let $\Delta\coloneqq A_{L} \oplus \mathscr{D}^{-1} $ be the maximal $A_{L}$-lattice in $H$.
    \item Let $N_{L / \Q_p}$ be the norm of the extension $L$.
\end{itemize}

Now \cite{hanke} describes the two isomorphism classes of such hermitian spaces over local fields. These are classified by their discriminant, which is an element of $\Q_p^\times /N_{L / \Q_p}(L^\times)$. For each class of $\Q_p^\times /N_{L / \Q_p}(L^\times)$, we pick a representative $\alpha \in \Z_p$ of minimal valuation, thus $0\leq v_p(\alpha) \leq 1$: 
\begin{itemize}
    \item In the odd case, $q=2m+1$, the two isomorphism classes look as follows: \\
For $\alpha \in \Q_p^\times$ let $V_\alpha\coloneqq H^m \oplus E_{\alpha}$, where $E_{\alpha}$ is the one dimensional hermitian space with hermitian form $h(x,y)=\alpha x \overline{y}$.\\
Now $\mathrm{disc}(h)=(-1)^m \alpha$. 
We define the corresponding maximal lattice 
$$
\Lambda_{\alpha}\coloneqq \Delta^m \oplus A_{L} 
$$

For both classes, the corresponding unitary groups are isomorphic, since we can switch between the classes by multiplying $S_h$ with an element of $\Q_p^\times$, leaving the unitary group invariant. Moreover, both groups are quasi-split.  
\item In the even case, $q=2m$, the two isomorphism classes look as follows: \\
For $\alpha \in N_{L / \Q_p}(L^\times)$ let $V_\alpha\coloneqq H^m$ and the maximal lattice
$$
\Lambda_{\alpha}=\Delta^m.
$$

Now $\mathrm{disc}(h)=(-1)^m= (-1)^m \alpha \in \Q_p^\times /N_{L / \Q_p}(L^\times)$. \\
For $\alpha \not\in N_{L / \Q_p}(L^\times)$ let $V_\alpha\coloneqq H^{m-1} \oplus D$, where $D$ is the division algebra $L \oplus L\cdot z$ over $\Q_p$ with the multiplication
\begin{align} 
    z^2 &= \alpha,    \nonumber \\ 
    x \cdot z &= z \cdot \overline{x}.
\end{align}
Let $A_D$ be its ring of integers and take the hermitian form 
\begin{align} \label{hermitian}
    h(x_1+x_2 \cdot z, y_1 + y_2 \cdot z)=x_1 \overline{y_1} - \alpha x_2 \overline{y_2}.
\end{align}

In this case, $\Lambda_{\alpha}=\Delta^{m-1} \oplus A_D$ and 
$\mathrm{disc}(h)=(-1)^{m} \alpha$. 
Here, only the unitary group attached to $V_\alpha$ for $\alpha \in N_{L / \Q_p}(L^\times)$ is quasi-split. 

\end{itemize}
With this classification of hermitian spaces over local fields, we make the following observations: If $n$ is even, every $\mathrm{G}(\Q_p)$ is quasi-split and hence $T_\ell=\emptyset$. For $n$ odd, we distinguish two cases: If $p$ is unramified, every unit is a norm, which implies that our global hermitian form over $\ell$ (with discriminant $-1$) descends to the local hermitian space corresponding to the identity in $N_{L / \Q_p}(L^\times)$, which is quasi-split (hence $p\not\in T_\ell$). If $p$ is ramified, denote by $\mathfrak{p}$ the unique prime ideal that lies above $p$. Then $p\in T_\ell$ if and only if $-1=\mathrm{disc}(h_{\mathrm{G}(\Q_p)})\neq \mathrm{disc}(h_{\mathscr{G}(\Q_p)})=(-1)^{\frac{n+1}{2}}$ in $\Q_p^\times / N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times)$, so that is the places where $(-1)^{\frac{n-1}{2}} \not\in N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times)$. This means that we can rewrite the product in (\ref{pra}) as in \cite[Section 3.1]{emery}:
\begin{align}
    \prod_p \frac{p^{\frac{1}{2}(\dim(\overline{M}_p) + \dim(\overline{\mathscr{M}}_p))}}{|\overline{M}_p(\mathbb{F}_{p})|} = 
    \prod_p \frac{p^{\dim(\overline{\mathscr{M}}_p)}}{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|} \cdot \prod_{p\in T_\ell} \lambda_p,
\end{align}
with 
\begin{align}
    \lambda_p=p^{\frac{1}{2}(\dim(\overline{M}_p) - \dim(\overline{\mathscr{M}}_p))} \frac{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|}{|\overline{M}_p(\mathbb{F}_{p})|}.
\end{align}

\subsection{The reductive quotients}
Let us determine the groups ${\overline{\mathscr{M}}}_p(\mathbb{F}_{p})$ in every case and $\overline{M}_p(\mathbb{F}_{p})$ for $p\in T_\ell$.
We go through the cases:
\begin{enumerate}
    \item \underline{$n$ even:}
    \begin{enumerate}
        \item \underline{$p$ is split in $\ell$:} \\
    If $p$ is split in $\ell$, we have $\mathrm{G}(\Q_p) \cong \mathrm{SL}(n+1)(\Q_p)$ and $\overline{\mathscr{M}}_p(\mathbb{F}_p)\cong \mathrm{SL}(n+1)(\mathbb{F}_p)$. 
    \item\label{even-unram} \underline{$p$ is inert in $\ell$:}\\
    Here ($p$ is unramified in $\ell$) $\overline{\mathscr{M}}_p(\mathbb{F}_p)\cong \mathrm{SU}(n+1)(\mathbb{F}_p)$, corresponding to the vertex $r=n$ in \cite[3.11]{tits}
    \item \underline{$p$ is ramified in $\ell$:}\\
    $\overline{\mathscr{M}}_p(\mathbb{F}_p)  \cong \mathrm{\mathrm{SO}}(n+1)(\mathbb{F}_p)$, again by  \cite[3.11]{tits}.
    \end{enumerate}
    \item \underline{$n$ odd:}
    \begin{enumerate}
        \item \underline{$p$ is split in $\ell$:}\\
    Again $\mathrm{G}(\Q_p) \cong \mathrm{SL}(n+1)(\Q_p)$ and $\overline{\mathscr{M}}_p(\mathbb{F}_p)\cong \mathrm{SL}(n+1)(\mathbb{F}_p)$. 
    \item \underline{$p$ is inert in $\ell$:}\\
     As in \cite[Table 2]{hanke} (again we only consider $\alpha = \pm 1$ and the Bruhat-Tits building is the same as for the unitary group considered there) we see that $\overline{\mathscr{M}}_p(\mathbb{F}_p)\cong \mathrm{SU}(n+1)(\mathbb{F}_p)$.
    \item \underline{$p$ is ramified in $\ell$, $-1 \in N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times)$:}\\
    $\overline{\mathscr{M}}_p(\mathbb{F}_p)\cong \mathrm{Sp}(n+1)(\mathbb{F}_p)$ (compare \cite[Table 2]{hanke}).
    \item \underline{$p$ is ramified in $\ell$, $-1 \not\in N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times)$:}\\
    Again $\overline{\mathscr{M}}_p(\mathbb{F}_p)\cong \mathrm{Sp}(n+1)(\mathbb{F}_p)$. However (\cite[Proposition 3.9]{hanke}),  
                        \begin{align*}
                            \overline{M}(\mathbb{F}_p) &= \{\mathrm{diag}(X,Y)|X\in \mathrm{Sp}(n-1)(\mathbb{F}_p), Y\in  \mathrm{O}^-(2)(\mathbb{F}_p), \det (Y)=1 \} \\
                        &\cong \mathrm{Sp}(2m-2)(\mathbb{F}_p) \times \mathrm{SO}^-(2)(\mathbb{F}_p), 
                        \end{align*}
    if $p$ is odd, where $\mathrm{SO}^-(2)$ is defined in \cite{finiteclassical2} 2.6. For $p=2$, the matrices in $\mathrm{O}^-(2)(\mathbb{F}_p)$ already have determinant $1$ and so 
    \begin{align*}
                            \overline{M}(\mathbb{F}_2) 
                        &\cong \mathrm{Sp}(2m-2)(\mathbb{F}_2) \times \mathrm{O}^-(2)(\mathbb{F}_2).
                        \end{align*}
         For $p\not\in T_\ell$ we have 
\begin{align*}
    \lambda_p &=p^{\frac{1}{2}(\dim(\mathrm{Sp}(n-1)\times \mathrm{SO}^-(2)) - \dim(\mathrm{Sp}(2m))} \frac{|\mathrm{Sp}(n+1)(\mathbb{F}_{p})|}{|\mathrm{Sp}(n-1)\times \mathrm{SO}^-(2)(\mathbb{F}_{p})|}= \\
    &= \frac{p^{n+1}-1}{p+1},
\end{align*}
due to \cite[Remark 1.2.3]{finiteclassical} and \cite[2.6]{finiteclassical2}.
    \end{enumerate}
\end{enumerate}

                                          

\subsection{The Volume Formula}

We now may apply \cite[Theorem 3.7]{prasad} and \cite[Proposition 3.6]{emery} (note that we omit the Tamagawa number in the formula, since it is $1$ in our case anyways):
\begin{align}
    \mu_{EP}(\Gamma \backslash G)=\chi(\C \mathbb{P}^n) |D_{\ell}|^{s(n)} \left( \prod_{r=1}^n \frac{r!}{(2\pi)^{r+1}}\right) \cdot \prod_p \frac{p^{\dim(\overline{\mathscr{M}}_p)}}{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|} \cdot \prod_{p\in T_\ell} \lambda_p,
\end{align}
with the following notation:
\begin{enumerate}
    \item \begin{align} \label{s(n)}
        s(n)= \left\{ \begin{matrix} 
    \frac{n(n+3)}{4}  &n\ even\\
    \frac{(n-1)(n+2)}{4}  &n \ odd.
    \end{matrix}\right.
    \end{align}
    \item $\mu_{EP}$ is the Euler-Poincare Measure on $G$
    \item $\chi(\C \mathbb{P}^n)$ is the Euler-Characteristic of the compact dual $U/K=\C \mathbb{P}^n$ of $G$.
 \end{enumerate}
To determine $\vol(\Gamma \backslash G)$ with the measure chosen above, we proceed as in \cite[proof of Proposition 4.1]{Harald} and use the fact that
\begin{align}
\mathrm{vol}_{\mu} &= \mathrm{vol}_{g_0}(\C \mathbb{P}^n) \frac{\mathrm{vol}_{EP}}{\chi(\C \mathbb{P}^n)} \\
 &= \mathrm{vol}_{g_0}(\C \mathbb{P}^n) \cdot |D_\ell|^{s(n)} \left( \prod_{r=1}^n \frac{r!}{(2\pi)^{r+1}}\right) \cdot \prod_{p} \frac{p^{\dim(\overline{\mathscr{M}}_p)}}{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|} \cdot \prod_{p \in T_\ell} \lambda_p,
\end{align}
where $\C \mathbb{P}^n$ is the compact dual of $G$, $g_0$ denotes the canonical Riemannian metric on $\C \mathbb{P}^n$.
We have 
$$
\overline{\mathscr{M}}_p= \left \{
\begin{matrix}
\mathrm{SL}(n+1)  & p \  split \\
\su(n+1)  & p \ inert \\
\mathrm{Sp}(n+1)  & p \ ramified
\end{matrix}\right.
$$
if $n$ is odd and 
$$
\overline{\mathscr{M}}_p= \left \{
\begin{matrix}
\mathrm{SL}(n+1)  & p \  split \\
\su(n+1)  & p \ inert \\
\mathrm{SO}(n+1)  & p \ ramified
\end{matrix}\right.
$$
if $n$ is even.
Thus (\cite[Remark 1.2.3]{finiteclassical} and \cite[2.6]{finiteclassical2}):
$$
\frac{p^{\dim(\overline{\mathscr{M}}_p)}}{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|} =  \left \{
\begin{matrix}
\prod_{i=2}^{n+1} \frac{1}{1-\frac{1}{p^i}} & p \  split \\
\prod_{i=2}^{n+1} \frac{1}{1-\frac{(-1)^i}{p^i}} & p \ inert \\
\prod_{i=1}^{\frac{n+1}{2}} \frac{1}{1-\frac{1}{p^{2i}}}  & p \ ramified.
\end{matrix}\right.
$$
This shows that 
\begin{align} \label{zetaproductodd}
   \prod_{p} \frac{p^{\dim(\overline{\mathscr{M}}_p)}}{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|}  =
   \zeta(2)L_\ell(3)\cdot ...\cdot \zeta(n+1),
\end{align}
if $n$ is odd,
where $L_\ell(s)$ is the Dirichlet L-Function attached to the field $\ell$. It is either defined as $\frac{\zeta_\ell}{\zeta}$ where $\zeta_\ell$ is the Dedekind zeta function attached to $\ell$, or as the L-function $L(s,\chi)$ where $\chi$ is the Jacobi symbol.\\
Analogously, we get 
\begin{align} \label{zetaproducteven}
   \prod_{p} \frac{p^{\dim(\overline{\mathscr{M}}_p)}}{|\overline{\mathscr{M}}_p(\mathbb{F}_{p})|}  =
   \zeta(2)L_\ell(3)\cdot ...\cdot L_\ell(n+1),
\end{align}
if $n$ is even.


By \cite[Equation 3.7]{vol}, we have

$$
\mathrm{vol}_{g_0}(\C \mathbb{P}^n)=\frac{\pi^n}{n!}.
$$ 
We combine these results to
\begin{thm} \label{volume-final}
$$
\vol (\Gamma \backslash G)= \pi^n |D_\ell|^{\frac{(n-1)(n+2)}{4}} \left( \prod_{i=1}^n \frac{(i-1)!}{(2\pi)^{i+1}}\right) \cdot \zeta(2)L_\ell(3)\cdot ...\cdot \zeta(n+1) \cdot \prod_{p \in T_\ell}\frac{p^{n+1}-1}{p+1} ,
$$
for $n$ odd and
$$
\vol (\Gamma \backslash G)= \pi^n |D_\ell|^{\frac{n(n+3)}{4}} \left( \prod_{i=1}^n \frac{(i-1)!}{(2\pi)^{i+1}}\right) \cdot \zeta(2)L_\ell(3)\cdot ...\cdot L_\ell(n+1),
$$
for $n$ even.
\end{thm}



==> 4Error.tex <==
\section{The Error Term} \label{error}



Recall that we intend to look at normal subgroups $\Gamma(m)$ of $\Gamma$ of finite index. We have to define what we mean by the principal congruence subgroups $\Gamma(m)$. \\
We defined the $\Q$-algebraic group $\mathrm{G}=\mathrm{SU}(n,1)$ as the unitary group of the hermitian form with signature $(n,1)$ over the imaginary field extension $\ell=\Q(\sqrt{-k})$.
\begin{align*}
    \mathrm{G}(\Q)= \left\{ X\in M_{n+1}(\ell)|\ X^\dagger S_{n,1} X= S_{n,1}, \det(x)=1 \right\}.
\end{align*}
By restriction of scalars of the field $\ell$, we may embed $\varphi: \mathrm{G}(\Q) \hookrightarrow \mathrm{GL}_{2(n+1)}(\Q)$. Set 
$$
\mathrm{G}_{\Z}\coloneqq\varphi^{-1} (\mathrm{GL}_{2(n+1)}(\Z)).
$$
This depends on the embedding $\varphi$, but the commensurability class of $\mathrm{G}_{\Z}$ does not. Let $m$ be coprime to $2k$ and define 
$$
\pi_m:\mathrm{GL}_{2(n+1)}(\Z) \twoheadrightarrow \mathrm{GL}_{2(n+1)}(\Z / m \Z )
$$
the reduction modulo $m$ map. 
%Let $n$ now be even. Then $\mathrm{G}$ is quasi-split over every local field $\Q_p$, by \cite[§2.1]{emery}.
We defined the arithmetic nonuniform lattice $\Gamma$ in the real group $G$ and computed its co-volume. This $\Gamma$ is commensurable with $\mathrm{G}_{\Z}$ \cite{emery}.
\begin{de} \label{congruence-subgroup}
We denote with
$$
\Gamma(1)\coloneqq\Gamma \cap \mathrm{G}_{\Z}
$$
be the congruence subgroup that has finite index in both $\Gamma$ and $G(\Z)$. 
Let
$$
\Gamma(m)\coloneqq\Gamma(1) \cap \ker ((\pi_m\circ \varphi)|_{\mathrm{G}_{\Z}}),
$$
for $m\geq 3$.
\end{de}
This implies that $\Gamma(m)$ is normal in $\Gamma(1)$. Furthermore, since $m\geq 3$, the group $\Gamma(m)$ is torsion free \cite[Lemma 1]{serre}.
Now we know that 
$$
\mathrm{vol}(\Gamma(m) \backslash G) = h_m\cdot  \mathrm{vol}(\Gamma \backslash G),
$$
where $h_m$ is the index of $\Gamma(m)$ in $\Gamma$. 


\subsection{Notations}

In the last chapter, we got a closed formula for $m(\Gamma(m),\pi)$ for the case that $n$ is odd. For $n$ even, we have to evaluate the error term 

\begin{align} \label{errror}
  \kappa (-1)^{n(\tau)} \dim (E_{\tau-\delta_K}) \cdot \sum_{i=1}^s \frac{\mathrm{vol}(\Gamma(m) \cap M^i \backslash M^i)}{\mathrm{vol}(\Gamma(m)\cap M_2^i \backslash M_2^i)^{n}}
\end{align}
in \ref{multiplicity}, where $M^i=\mathrm{R}_u(Q^i)$ are the unipotent radicals of the cusps $Q^1,...,Q^s$ of $\Gamma(m)$.
The proof of Theorem 10 in \cite{degeorge} gives the following:
$$
\sum_{i=1}^s \frac{\mathrm{vol}(\Gamma(m) \cap M^i \backslash M^i)}{\mathrm{vol}(\Gamma(m)\cap M_2^i \backslash M_2^i)^{n}}=h_N \sum_{j=1}^r \frac{\mathrm{vol}(\Gamma(1) \cap N^j \backslash N^j)}{\mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j)^{n}},
$$
where $N^j=\mathrm{R}_u(
P^j)$ for the cusps $P^1,...,P^r$ of $\Gamma(1)$. So we have to determine $\mathrm{vol}(\Gamma(1) \cap N^j \backslash N^j)$ and $\mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j)$ or at least give an upper bound for the quotient. %We will make the parabolic subgroup $P_0$, as defined in section \ref{prelims}, explicit. \\
 We introduce the notation
 $$
 A(a,b)\coloneqq\left(\begin{matrix}
a & 0 & ... & b \\
0 & 1 & ... & 0 \\
... & & & \\
b & 0 & ... & a
 \end{matrix}\right),
 $$
 so $A=\{A(a,b)|\ a,b\in\R\}$. \\
 Now 
 $$
 N_2=\mathrm{exp}(\mathfrak{g}_2)=\{u_2(\mu)|\ \mu\in\R\}, 
 $$
 where 
 $$
 u_2(\mu)\coloneqq\left(\begin{matrix}
1-i\mu & 0 & ... & i\mu \\
0 & 1 & ... & 0 \\
... & & & \\
-i\mu & 0 & ... & 1+i\mu
 \end{matrix}\right)
 $$
 and 
 $$
 N=\mathrm{exp}(\mathfrak{g}_1 \oplus \mathfrak{g}_2)=\{u(\mathbf{x},\mu)|\ \mu\in\R,\ \mathbf{x}=(x_1,...,x_{n-1})\in \C^{n-1} \}, 
 $$
 where 
 $$
u(\mathbf{x},\mu)\coloneqq u_2(\mu) + \left(\begin{matrix}
-\frac{|\mathbf{x}|^2}{2} & x_1 & x_2 & ... & \frac{|\mathbf{x}|^2}{2} \\
-\overline{x_1} & 0 & 0 & ... & \overline{x_1} \\
...& & & & \\
-\frac{|\mathbf{x}|^2}{2} & x_1 & x_2 & ... & \frac{|\mathbf{x}|^2}{2}
 \end{matrix}\right).
 $$
 Above, we have set
 $$
 |\mathbf{x}|^2\coloneqq\langle \mathbf{x},\mathbf{x}\rangle,
 $$
 where
 $$
 \langle \mathbf{x}, \mathbf{y} \rangle \coloneqq \sum_{i=1}^{n-1} x_i\overline{y_i}. 
 $$
 Note that 
 $$
 u_2(\mu_1)\cdot u_2(\mu_2)=u_2(\mu_1+\mu_2)
 $$
 and 
 $$
 u(\mathbf{x}^1,\mu_1)\cdot  u(\mathbf{x}^2,\mu_2) = 
 u(\mathbf{x}^1+\mathbf{x}^2, \mu_1+\mu_2+\mathrm{Im}(\langle \mathbf{x}^1,\mathbf{x}^2\rangle )).
 $$
\\
In Section \ref{prelims}, we defined $M$ as the centralizer of $A$ in $K$. This means, that 
\begin{align*}
    M &=\{X\in K|\ A(a,b)X=XA(a,b)\ \forall a,b\in \R\}\\
    &= \{\mathrm{diag}(e^{i\theta},Y,e^{i\theta})|\ Y^\dagger Y= 1,\ \det(Y)=e^{-2i\theta}  \}.
\end{align*}
We have $P_0=MAN$. Recall that we sum the Error terms 
$$
\frac{\mathrm{vol}(\Gamma(1) \cap N^j \backslash N^j)}{\mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j)^{n}},
$$
where $j$ runs through an indexation $P^1,...,P^r$ of the cusps of $G$ (that is, $\Gamma(1)$-conjugacy classes of $\Gamma(1)$-cuspidal parabolic subgroups of $G$). For an arbitrary $P^i\in P_\Gamma$, we have that 
\begin{align*}
    P^i&=M^iA^iN^i \\
    N^i&=k_i^{-1} N k_i \\
    N_2^i &= k_i^{-1} N_2 k_i, 
\end{align*}
where $k_i\in K$. 
\subsection{Estimating the error term}
Assume we work with $n$ even, the only case where the error terms appear. Here, we know that there is only one commensurability class of nonuniform arithmetic lattices.
We want to estimate the size of $\mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j)$.
    We know that $N_2^j=(k^j)^\dagger N_2 k^j$, for some $k^j\in K$. Now let 
    $$
    k^j= \left(\begin{matrix}
        k_{11} & k_{12} & \ldots & 0 \\
        k_{21} & k_{22} & \ddots & 0 \\
        \vdots & \vdots & \ddots & 0 \\
        0 & 0& \ldots & k_{n+1,n+1}
    \end{matrix}\right).
    $$
    Then an element of $\Gamma(m) \cap N_2^j$ is of the form $u_2^j(\mu)\coloneqq(k^j)^\dagger u_2(\mu)k^j$ and its $(n+1,n+1)$-entry is still $1 + i \mu$. But this implies that $\mu = \sqrt{k} zm$ for $z \in \Z$. We thus see that 
    $\Gamma(m) \cap N_2^j \subseteq \{u_2^j(\sqrt{k} mz)| z\in \Z\}\subseteq N_2^j$ and so
\begin{align} \label{volume-N2}
    \mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j) &\geq \mathrm{vol}(\{u_2^j(\sqrt{k} mz)| z\in \Z\} \backslash N_2^j)\nonumber\\
    &=\mathrm{vol}(\{u_2(\sqrt{k} mz)| z\in \Z\} \backslash N_2) 
    = \sqrt{\frac{k}{8(n+1)}} m,
\end{align}
with the normalization of the Haar measure chosen in Section \ref{prelims}.
    



We plug this into the error term (\ref{errror}) and get:

\begin{align*}
 & \left| \kappa (-1)^{n(\tau)} \dim (E_{\tau-\delta_K}) \cdot \sum_{i=1}^s \frac{\mathrm{vol}(\Gamma(m) \cap M^i \backslash M^i)}{\mathrm{vol}(\Gamma(m)\cap M_2^i \backslash M_2^i)^{n}} \right|\\
\leq & |\kappa| \dim (E_{\tau-\delta_K}) \cdot h_m \sum_{j=1}^r \frac{\mathrm{vol}(\Gamma(1) \cap N^j \backslash N^j)}{\mathrm{vol}(\Gamma(m)\cap N_2^j \backslash N_2^j)^{n}} \\
\leq  & |\kappa|  \dim (E_{\tau-\delta_K}) \cdot \frac{h_m}{\left(\sqrt{\frac{k}{8(n+1)}} m \right)^n}\sum_{j=1}^r \mathrm{vol}(\Gamma(1) \cap N^j \backslash N^j) \\
\eqqcolon  & C \frac{h_m}{m^n}.
\end{align*}
When we note that 
$$
\mathrm{vol}(\Gamma(m) \backslash G) = h_{m}\cdot \mathrm{vol}(\Gamma \backslash G),
$$
we obtain our main result:

\begin{thm} \label{mult}
Let $\Gamma$ be an arithmetic subgroup of $G=SU(n,1)$ as in Definition \ref{defgamma} and let $\Gamma(m)$ be a principal congruence subgroup (as in Definition \ref{congruence-subgroup}) of index $h_m$ in $\Gamma$, with $n\geq 3$ and $m\geq 3$. Let $\pi_\tau \in \hat{G}$ be of integrable discrete series with Harish-Chandra parameter $\tau=(\tau_1,.\ldots,\tau_n)_{\{\varepsilon_i\}}$ with $\tau_{n+1}\ceq - \sum_{i=1}^n \tau_i$, where
\begin{align*}
        \tau_1 &> \tau_2 > \ldots >\tau_n > \tau_{n+1}+n.
        \end{align*}
Then we have
\begin{align*}
    &m(\Gamma(m),\pi_\tau) =d_\tau \mathrm{vol}(\Gamma  \backslash G)h_m \\
    &= \frac{h_m}{4^n} \prod_{i=1}^n  \frac{\left|\prod_{j=i+1}^{n+1} (\tau_i-\tau_j)\right|}{(2\pi)^{i+1}} 
    \cdot |D_\ell|^{\frac{(n-1)(n+2)}{4}}  \cdot \zeta(2)L_\ell(3)\cdot ...\cdot \zeta(n+1) 
    \cdot \prod_{p \in T_\ell}\frac{p^{n+1}-1}{p+1} 
\end{align*}
if $n$ is odd and 
\begin{align*}
&m(\Gamma(m),\pi_\tau) =d_\tau \mathrm{vol}(\Gamma  \backslash G)h_m + O\left( \frac{h_m}{m^n}\right) \\
&= h_m \left( \frac{1}{4^n} \prod_{i=1}^n  \frac{\left|\prod_{j=i+1}^{n+1} (\tau_i-\tau_j)\right|}{(2\pi)^{i+1}} \cdot |D_\ell|^{\frac{n(n+3)}{4}}  \cdot \zeta(2)L_\ell(3)\cdot ...\cdot L_\ell(n+1) + O\left( \frac{1}{m^n}\right)\right)
\end{align*}
if $n$ is even.
The set $T_\ell$ consists of those ramified primes $p=\mathfrak{p}^2$ in $\ell$, where $(-1)^{\frac{n-1}{2}} \not\in N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times).$
\end{thm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse



\subsection{Error term alternative}
Some of the volumes above can be even made more explicit.
We begin with computing $\mathrm{vol}(G(\Z) \cap N \backslash N)$.
With the notation $\mathbf{x}=(x_1+\sqrt{-k}y_1,...,x_{n-1}+\sqrt{-k}y_{n-1})$ we have
    $$
    G(\Z) \cap N= \{N(\mathbf{x},\mu)|\ x_i,y_i\in \Z\ \forall i\leq n-1, \mu\in\Z,\ 2||\mathbf{x}|^2\} 
    $$
    A fundamental domain is
    $$
    D\coloneqq\{ N(\mathbf{x},\mu)|\ x_i\in [0,1)\ for\ i\leq n-1,\ y_i\in [0,\sqrt{k})\ for\ i\leq n-2,\ y_{n-1}\in [0,2\sqrt{k}),\  \mu\in[0,\sqrt{k})\}
    $$
    and thus
    $$
    \mathrm{vol}(G(\Z) \cap N \backslash N)= 2K^{\frac{2n-1}{2}}\sqrt{k}^{n}.
    $$
    Since 
    $$
    G(\Z) \cap N_2 = \{N_2(\mu)|\ \mu\in\Z\}, 
    $$
    we have
    $$
    \mathrm{vol}(G(\Z) \cap N_2 \backslash N_2)= K^{\frac{1}{2}}.
    $$
    Now for ${\mathrm{vol}(G(\Z)\cap N_2^j \backslash N_2^j)^{n}}$, we know that $N_2^j=(k^j)^\dagger N_2 k^j$, for some $k^j\in K$. Now let 
    $$
    k^j= \left(\begin{matrix}
        k_{11} & k_{12} & \ldots & 0 \\
        k_{21} & k_{22} & \ddots & 0 \\
        \vdots & \vdots & \ddots & 0 \\
        0 & 0& \ldots & k_{n+1,n+1}
    \end{matrix}\right).
    $$
    Then $(k^j)^\dagger N_2(\mu)k^j= $
    $$
    \left(\begin{matrix}
        -k_{11}\overline{k_{11}} & -k_{12}\overline{k_{11}} & \ldots & -k_{n+1,n+1}\overline{k_{11}} \\
        -k_{11}\overline{k_{12}} & -k_{12}\overline{k_{22}} & \ddots & -k_{n+1,n+1}\overline{k_{1n}} \\
        \vdots & \vdots & \ddots & -k_{n+1,n+1}\overline{k_{1,n}} \\
        -k_{11}\overline{k_{n+1,n+1}} & -k_{12}\overline{k_{n+1,n+1}}& \ldots & 1
    \end{matrix}\right).
    $$
    If we let $k_0^j$ be the minimal integer such that 
    $$
    k_0^j\cdot a\overline{b} \in \Z\ \forall a,b\in \{k_{11},k_{12},...,k_{n+1,n+1}\},
    $$
    then $(k^j)^\dagger N_2(\mu)k^j\in G(\Z)\cap N_2^j$ implies that $\mu\in\Z$ and $k_0^j|\mu$. We can deduce that 
    $$
    \mathrm{vol}(G(\Z) \cap N_2^j \backslash N_2^j)= k_0^j\cdot K^{\frac{1}{2}}.
    $$
    We have 
    $$
\mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j) = [\Gamma(m) \cap N_2^j : G(\Z) \cap N_2^j  ] \cdot  \mathrm{vol}(G(\Z) \cap N_2^j \backslash N_2^j),
$$
and the index $[\Gamma(m) \cap N_2^j : G(\Z) \cap N_2^j  ]$ is finite because of the second isomorphism theorem. 
Now we do an analogous thing as above, but for the group $\ker (\pi_N|_{G(\Z)})$ and see that 
$$
\mathrm{vol}(\Gamma(m) \cap N_2^j \backslash N_2^j) = [\Gamma(m) \cap N_2^j : \ker (\pi_N|_{G(\Z)}) \cap N_2^j  ] \cdot  \mathrm{vol}(\ker (\pi_N|_{G(\Z)}) \cap N_2^j \backslash N_2^j),
$$
where 
$$
\mathrm{vol}(\ker (\pi_N|_{G(\Z)}) \cap N_2^j \backslash N_2^j)=k_0^j\cdot K^{\frac{1}{2}}N
$$
and we set 
$$
h_2^j(N)\coloneqq [\Gamma(m) \cap N_2^j : \ker (\pi_N|_{G(\Z)}) \cap N_2^j  ] = \color{red} [\Gamma(m):\ker (\pi_N|_{G(\Z)})]? \color{black}.
$$


\fi

==> 5Growth.tex <==
\section{Application I: Cuspidal Cohomology} \label{cuspcoh}

As before, we let $\tau=\lambda + \delta_G$. In Theorem 5.3 of \cite{zuck}, the $\mathfrak{g}$-module $A_{\mathfrak{q}}(\lambda)$ is identified as the discrete series representation of Harish-Chandra parameter $\tau$, if we let $\mathfrak{q}$ be the standard parabolic sub-algebra of $\mathfrak{g}$ corresponding to the parabolic subgroup $P$ of $G$, given by the upper triangular matrices in $G$. We require 
    \begin{align*}
        (\lambda,\alpha)\geq 0\ \forall \alpha \in \Delta_G^+,
    \end{align*}
    which is equivalent to 
    \begin{align} \label{cohom-condition}
        \tau_i +i &\geq \tau_j + j \quad \ &for\  1\leq i <j\leq n, \nonumber \\
        \tau_i  &\geq  \tau_{n+1} + \frac{n(n+1)}{2} + n+1 -i \quad \ &for\  1\leq i \leq n,
    \end{align}
    where again we have set $\tau_{n+1} = -\sum_{i=1}^n \tau_i $.
    According to Theorem 5.3 and Theorem 5.5 in \cite{zuck} we have that $\pi_\tau$ is cohomological with respect to $F_{\lambda}$,
    the finite dimensional irreducible representation of $\mathfrak{g}$ of lowest weight $-\lambda$. \\ 
    More precisely, we have that (note that $\dim \mathfrak{u} \cap \mathfrak{p}=n$)
    \begin{align*}
        H^i(\mathfrak{g},\mathfrak{k},\pi_\tau \otimes F_{\lambda}) \cong H^{i-n}(\mathfrak{t},\mathfrak{t}\cap \mathfrak{k},\C) \cong \mathrm{Hom}_{\mathfrak{t}}(\Lambda^{i-n}(0),\C),
    \end{align*}
    which means that 
    \begin{align} \label{cohomology}
        H^i(\mathfrak{g},\mathfrak{k},\pi_\tau \otimes F_{\lambda}) \cong \left\{ 
        \begin{matrix}
            \C & if\ i=n \\
            0 & else.
        \end{matrix}
        \right.
    \end{align}
    Also, for $F \not \cong F_{\lambda}$, 
    \begin{align*}
        H^i(\mathfrak{g},\mathfrak{k},\pi_\tau \otimes F)= 0. 
    \end{align*}
    
 We have defined the arithmetic subgroup $\Gamma(1)$ of $G$ above. Consider a tower of arithmetic subgroups $\{\Gamma(m_i)\}_{i=1}^\infty$ of $G$, where $m_1=1$ and $\Gamma(m_i)$ is a normal congruence subgroup of finite index in $\Gamma(1)$, as in the previous section. We also assume 
$$
\bigcap_{i=1}^\infty \Gamma(m_i)=\{1\}. 
$$
With the notation from above, we get the following: 
\begin{thm} (Theorem 10 in \cite{degeorge}) \\
For $\pi_\tau$ of integrable discrete series, we have
$$
\lim_{i \rightarrow \infty} \frac{m(\Gamma(m_i),\pi_\tau)}{\mathrm{vol}(\Gamma(m_i) \backslash G)} = d_\tau.
$$

\end{thm}

With the estimates derived in the last chapter, we can give an explicit bound for this growth rate:
\begin{cor} \label{growth}
For $n$ odd, we have
\begin{align*}
    m(\Gamma(m_i),\pi_\tau) &= d_\tau \mathrm{vol}(\Gamma(m_i) \backslash G) \\
&=\frac{h_{m_i}}{4^n} \prod_{i=1}^n \frac{\left| \prod_{j=i+1}^{n+1} (\tau_i - \tau_j) \right|}{(2\pi)^{i+1}} \\
& \cdot |D_\ell|^{\frac{(n-1)(n+2)}{4}} \cdot \zeta(2)L_\ell(3)\cdot ...\cdot \zeta(n+1) \cdot \prod_{p \in T_\ell}\frac{p^{n+1}-1}{p+1}.
\end{align*}
For $n$ even:
\begin{align*}
    m(\Gamma(m_i),\pi_\tau) &\geq d_\tau \mathrm{vol}(\Gamma(m_i) \backslash G) - C \frac{h_{m_i}}{m_i^n} \\
&=\frac{h_{m_i}}{4^n} \prod_{i=1}^n \frac{\left| \prod_{j=i+1}^{n+1} (\tau_i - \tau_j) \right|}{(2\pi)^{i+1}}  \\
&\cdot |D_\ell|^{\frac{n(n+3)}{4}} \left( \prod_{r=1}^n \frac{1}{(2\pi)^{r+1}}\right) \cdot \zeta(2)L_\ell(3)\cdot ...\cdot L_\ell(n+1) - C\frac{h_{m_i}}{m_i^n}.
\end{align*}
\end{cor}
Here we have used  Theorem \ref{mult}.
This last equation for the even case shows that
$$
\frac{m(\Gamma(m_i),\pi) }{\mathrm{vol}(\Gamma(m_i) \backslash G)}\geq d_\tau - \frac{C}{ \mathrm{vol}(\Gamma \backslash G) m_i^n  },
$$
because 
$$
\mathrm{vol}(\Gamma(m_i) \backslash G) = h_{m_i}\cdot \mathrm{vol}(\Gamma \backslash G).
$$
In particular, this tells us that the multiplicity is strictly positive (that, of course, means non-zero) as soon as 
$$
m_i \geq \left|\frac{C}{d_\tau \mathrm{vol}(\Gamma \backslash G)} \right|^{\frac{1}{n}}.
$$
\color{black}
We want to apply this result to get some growth estimates of cuspidal cohomology.
Let $X\coloneqq G/K$ be the Riemannian symmetric space associated to $G$. For $m_i \geq 3$ we have that $\Gamma(m_i)$ is a torsion free arithmetic subgroup of $G$. Then 
$$
S(\Gamma(m_i))\coloneqq\Gamma(m_i) \backslash X
$$
is a locally symmetric space and a smooth, non-compact manifold of finite volume. Let $F_{\lambda}$ be the irreducible, finite dimensional representation of $G$ of lowest weight $-\lambda$.
We denote by $\Tilde{F_{\lambda}}$ the locally constant sheaf corresponding to $F_{\lambda}$. 
Recalling the definition of cuspidal cohomology (\cite[1.2]{Harald}), we have 
$$
H_{cusp}^* (S(\Gamma(m_i)),\Tilde{F_{\lambda}})\coloneqq H^*(\mathfrak{g},K,L_{cusp}^2(\Gamma(m_i) \backslash G)^\infty \otimes F_{\lambda}).
$$
Here $L_{cusp}^2(\Gamma(m_i) \backslash G)$ denotes the space of square integrable functions $f:\Gamma(m_i) \backslash G \rightarrow \C$ that are cuspidal, i.e.
$$
\int_{\Gamma(m_i) \cap N \backslash N} f(ng)\,\mathrm{d}n =0 \qquad for\ almost\ all\  g\in G,
$$
where $N$ denotes the unipotent radical of $G$. Now by \cite[Proposition 5.6]{laplacian} we have
$$
H_{cusp}^* (S(\Gamma(m_i)),\Tilde{F_{\lambda}})\coloneqq \bigoplus _{\pi \in \hat{G}_{coh}} H^*(\mathfrak{g},K,\pi_{(K)} \otimes F_{\lambda})^{m(\Gamma(m_i),\pi)}.
$$
Using Corollary \ref{growth} and Equation \ref{cohomology} we get the following:
\begin{thm} 
Let $\{\Gamma(m_i)\}_{i=1}^\infty$ be a tower of arithmetic subgroup of $G=SU(n,1)$, as above. Let $\pi_\tau \in \hat{G}$ be of integrable discrete series with Harish-Chandra parameter $\tau=\lambda + \delta_G$, where $\tau \in L_T'$ satisfies
 \begin{align*} 
        \tau_i +i &\geq \tau_j + j \quad \ &for\  1\leq i <j\leq n, \nonumber \\
        \tau_i  &\geq  \tau_{n+1} + \frac{n(n+1)}{2} + n+1 -i \quad \ &for\  1\leq i \leq n.
    \end{align*}
 Let $F_{\lambda}$ be the irreducible, finite dimensional representation of $G$ of lowest weight $-\lambda$ and denote by $\Tilde{F_{\lambda}}$ the locally constant sheaf attached to $F_{\lambda}$.
Then, for $n$ odd, we have
\begin{align*}
    \dim H_{cusp}^n (S(\Gamma(m_i)),\Tilde{F_{\lambda}}) & \geq  d_\tau \mathrm{vol}(\Gamma(m_i) \backslash G) \\
&=\frac{h_{m_i}}{4^n} \prod_{i=1}^n \frac{\left| \prod_{j=i+1}^{n+1} (\tau_i - \tau_j) \right|}{(2\pi)^{i+1}} \\
& \cdot |D_\ell|^{\frac{(n-1)(n+2)}{4}} \cdot \zeta(2)L_\ell(3)\cdot ...\cdot \zeta(n+1) \cdot \prod_{p \in T_\ell}\frac{p^{n+1}-1}{p+1}.
\end{align*}
For $n$ even:
\begin{align*}
    \dim H_{cusp}^n (S(\Gamma(m_i)),\Tilde{F_{\lambda}}) & \geq  d_\tau \mathrm{vol}(\Gamma(m_i) \backslash G) - C \frac{h_{m_i}}{m_i^n} \\
&=\frac{h_{m_i}}{4^n} \prod_{i=1}^n \frac{\left| \prod_{j=i+1}^{n+1} (\tau_i - \tau_j) \right|}{(2\pi)^{i+1}}  \\
&\cdot |D_\ell|^{\frac{n(n+3)}{4}} \left( \prod_{r=1}^n \frac{1}{(2\pi)^{r+1}}\right) \cdot \zeta(2)L_\ell(3)\cdot ...\cdot L_\ell(n+1) - C\frac{h_{m_i}}{m_i^n}.
\end{align*}
\end{thm}

==> 6Rational.tex <==
\section{Application II: Rationality of L-functions} \label{rationality}


As before, let $\ell=\Q(\sqrt{-k})$ be a quadratic extension, $D_\ell$ the corresponding discriminant and $L_\ell$ the corresponding $L$-function. It is also the $L$-function corresponding to the Jacobi-symbol of $\ell$ interpreted as a character which we denote by $\chi_\ell$ (i.e. $L_\ell(s)=L(s,\chi_\ell)$). Then:


\begin{cor} \label{rational}
Let $\ell=\Q(\sqrt{-k})$ be an imaginary quadratic quadratic field. Let $\Gamma^{(1)}$ and $\Gamma^{(2)}$ be the arithmetic subgroups as in Definition \ref{defgamma} of $SU(2n-1,1)$ and $SU(2n+1,1)$ respectively and let $\Gamma^{(i)}(m^{(i)})$ be the principal congruence subgroups (as in Definition \ref{congruence-subgroup}) of index $h_{m^{(i)}}$ in $\Gamma^{(i)}$, with $n\geq 2$ and $m^{(i)}\geq 3$. Let $\pi_{\tau^{(i)}} \in \hat{G}$ be the discrete series representation with Harish-Chandra parameter $\tau^{(i)}$, such that 
\begin{align*}
        \tau_i^{(1)} &= \tau_i^{(2)} \ for\ 1\leq i \leq 2n-1.,  \\
        \tau_1^{(1)} &> \tau_2^{(1)} > \ldots \tau_{2n-1}^{(1)}>\tau_{2n}^{(1)} +2n -1,\\
        \tau_{2n-1}^{(2)} &> \tau_{2n}^{(2)}> \tau_{2n+1}^{(2)} >\tau_{2n+2}^{(2)}+2n+1, 
        \end{align*}
where we set 
\begin{align*}
    \tau_{2n}^{(1)} &\ceq -\sum_{i=1}^{2n-1} \tau_i^{(1)}, \\
    \tau_{2n+2}^{(2)} &\ceq -\sum_{i=1}^{2n+1} \tau_i^{(2)}.
\end{align*}

This implies that $\pi_{\tau^{(i)}}$ is of integrable discrete series. Then
    \begin{align*}
    &\sqrt{|D_\ell|} \frac{L_\ell(2n+1)}{(2\pi)^{2n+1}} \\
      = &\frac{m(\Gamma^{(2)}(m^{(2)}),\pi_{\tau^{(2)}})}{m(\Gamma^{(1)}(m^{(1)}),\pi_{\tau^{(1)}})} \cdot \frac{32h_{m^{(1)}}}{h_{m^{(2)}}}  \frac{\displaystyle\prod_{\substack{1 \leq i <  2n \\ }} (\tau_i^{(1)}-\tau_{2n}^{(1)})}{\displaystyle \prod_{\substack{1 \leq i < j \leq 2n+2 \\ 2n \leq j}}(\tau_i^{(2)}-\tau_j^{(2)})}\\
      & \cdot \prod_{p \in T_\ell^{(1)}}\frac{p^{2n}-1}{p+1} \cdot \prod_{p \in T_\ell^{(2)}}\frac{p+1}{p^{2n+2}-1} |D_\ell|^{2n}  \frac{(2n+2)!}{(-1)^n B_{2n+2}},
    \end{align*}
    where the set $T_\ell^{(1)}$ (resp. $T_\ell^{(2)}$) consists of those ramified primes $p=\mathfrak{p}^2$ in $\ell$, where $(-1)^{n-1} \not\in N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times)$ (resp. $(-1)^{n} \not\in N_{\ell_{\mathfrak{p}} / \Q_p}(\ell_{\mathfrak{p}}^\times)$).
In particular, this implies that $\sqrt{|D_\ell|} \frac{L_\ell(2n+1)}{(2\pi)^{2n+1}}$ is a rational number.
\end{cor}
\begin{proof}
From Theorem \ref{mult} for the two cases $n \mapsto 2n-1$ and $n \mapsto 2n+1$, we can deduce (by dividing one equation by the other) that 
    \begin{align*}
        & \frac{m(\Gamma^{(2)}(m^{(2)}),\pi_{\tau^{(2)}})}{m(\Gamma^{(1)}(m^{(1)}),\pi_{\tau^{(1)}})}\\
        =  &\frac{h_{m^{(2)}}}{16h_{m^{(1)}}}  
        \frac{\displaystyle \prod_{\substack{1 \leq i < j \leq 2n+2 \\ 2n \leq j}}(\tau_i^{(2)}-\tau_j^{(2)})}{\displaystyle\prod_{\substack{1 \leq i <  2n \\ }} (\tau_i^{(1)}-\tau_{2n}^{(1)})}
    \cdot |D_\ell|^{\frac{4n+1}{2}} \\
    &\cdot \frac{L_\ell(2n+1)}{(2\pi)^{2n+1}}\cdot \frac{\zeta(2n+2) }{(2\pi)^{2n+2}}
    \cdot \prod_{p \in T_\ell^{(1)}}\frac{p+1}{p^{2n}-1} \cdot \prod_{p \in T_\ell^{(2)}}\frac{p^{2n+2}-1}{p+1}.
    \end{align*}
    We rearrange this to obtain the expression
    \begin{align*}
      &|D_\ell|^{\frac{1}{2}}  \frac{L_\ell(2n+1)}{(2\pi)^{2n+1}} \\
      = &\frac{m(\Gamma^{(2)}(m^{(2)}),\pi_{\tau^{(2)}})}{m(\Gamma^{(1)}(m^{(1)}),\pi_{\tau^{(1)}})} \cdot \frac{16 h_{m^{(1)}}}{h_{m^{(2)}}} \\
      & \cdot \frac{\displaystyle\prod_{\substack{1 \leq i <  2n \\ }} (\tau_i^{(1)}-\tau_{2n}^{(1)})}{\displaystyle \prod_{\substack{1 \leq i < j \leq 2n+2 \\ 2n \leq j}}(\tau_i^{(2)}-\tau_j^{(2)})} \prod_{p \in T_\ell^{(1)}}\frac{p^{2n}-1}{p+1} \cdot \prod_{p \in T_\ell^{(2)}}\frac{p+1}{p^{2n+2}-1}|D_\ell|^{2n}  \frac{(2\pi)^{2n+2}}{\zeta(2n+2) } 
    \end{align*}
    It is well known that 
    $$
    \zeta(2n+2)=(-1)^n \frac{(2\pi)^{2n+2}B_{2n+2}}{2(2n+2)!},
    $$
    where $B_n$ denotes the $n$-th Bernoulli number. 
   We can deduce that
    \begin{align*}
    &|D_\ell|^{\frac{1}{2}}  \frac{L_\ell(2n+1)}{(2\pi)^{2n+1}} \\
      = &\frac{m(\Gamma^{(2)}(m^{(2)}),\pi_{\tau^{(2)}})}{m(\Gamma^{(1)}(m^{(1)}),\pi_{\tau^{(1)}})} \cdot \frac{32h_{m^{(1)}}}{h_{m^{(2)}}}  \frac{\displaystyle\prod_{\substack{1 \leq i <  2n \\ }} (\tau_i^{(1)}-\tau_{2n}^{(1)})}{\displaystyle \prod_{\substack{1 \leq i < j \leq 2n+2 \\ 2n \leq j}}(\tau_i^{(2)}-\tau_j^{(2)})}\\
      & \cdot \prod_{p \in T_\ell^{(1)}}\frac{p^{2n}-1}{p+1} \cdot \prod_{p \in T_\ell^{(2)}}\frac{p+1}{p^{2n+2}-1} |D_\ell|^{2n}  \frac{(2n+2)!}{(-1)^n B_{2n+2}}.
    \end{align*}
    The expression on the right hand side only involves rational numbers, which implies that
    \begin{align} \label{rat}
        \sqrt{|D_\ell|} \frac{L_\ell(2n+1)}{(2\pi)^{2n+1}}\in \Q.
    \end{align}

\end{proof}

\begin{rmk}
    A possible choice for $\tau^{(i)}$ is for example
    \begin{align*}
        \tau_i^{(1)} & \ceq 2n+2-i &\ for\ i\leq 2n-1, \\
        \tau_i^{(2)} &\ceq 2n+2 -i  &\ for\ i\leq 2n+1. 
    \end{align*}
    in which case we have 
    \begin{align*}
        \frac{\displaystyle\prod_{\substack{1 \leq i <  2n \\ }} (\tau_i^{(1)}-\tau_j^{(1)})}{\displaystyle \prod_{\substack{1 \leq i < j \leq 2n+2 \\ 2n \leq j}}(\tau_i^{(2)}-\tau_j^{(2)})} = \frac{\displaystyle\prod_{\substack{1 \leq i <  2n \\ }} (2n-i+2+(n+2)(2n-1))}{\displaystyle (2n-1)! (2n)!\prod_{\substack{1 \leq i \leq 2n+1}}(2n+2-i+(n+1)(2n+1))} \\
        =  \frac{1}{(2n-1)! (2n)!(2n^2+3n+2)} \prod_{\substack{1 \leq i <  2n \\ }} \frac{2n^2+5n-i}{2n^2+5n+3-i}. 
    \end{align*}
\end{rmk}



The rationality result (\ref{rat}) is already known, but the usual way to prove it is the following:


In \cite{Siegel}, Siegel showed that 
\begin{align*}
    L(1-n,\chi_\ell) \in \Q,\ for\ n\geq 1
\end{align*}
for real quadratic fields $\ell$. For imaginary quadratic fields $\ell$, the same is true due to \cite[Theorem 4.2]{wash}.


Now from \cite[Theorem 12.11]{apo} we have the functional equation 
\begin{align*}
    L(1-s,\chi)=\frac{k^{s-1}\Gamma(s)}{(2\pi)^s}\left( e^{-\frac{i\pi s}{2}} +\chi(-1) e^{\frac{i \pi s}{2}} \right) G(1,\chi) L(s,\overline{\chi}),
\end{align*}
where $\chi$ is a primitive character modulo $k$, $s\in \R$ and $G(m,\chi)$ is the Gauss sum 
\begin{align*}
    \sum_{r=1}^k \chi(r) e^{\frac{2 \pi i rm}{k}}.
\end{align*}
Since $\chi_\ell$ is a real character and primitive, we have $\overline{\chi_\ell}= \chi_\ell$ and $k=|D_\ell|$. Hence
\begin{align*}
    L(-2m,\chi_\ell) & =\frac{|D_\ell|^{2m}\Gamma(2m+1)}{(2\pi)^{2m+1}} (-1)^m \left( e^{-\frac{i\pi}{2}} - e^{\frac{i \pi }{2}} \right) G(1,\chi_\ell) L(2m+1,\chi_\ell)  \Leftrightarrow \\
   \frac{(-1)^{m}}{2|D_\ell|^{2m} (2m)! } L(-2m,\chi_\ell) & = \frac{-i G(1,\chi_\ell) L_\ell(2m+1)}{(2\pi)^{2m+1}}.
\end{align*}

To evaluate $G(1,\chi_\ell)$, we note that $|G(1,\chi_\ell)|^2=|D_\ell|$ due to \cite[Theorem 8.15]{apo} and we have that 
\begin{align*}
    \overline{G(1,\chi_\ell)} &= \sum_{r=1}^{|D_\ell|-1} \chi_\ell(r) e^{-\frac{2\pi i r}{|D_\ell|}} = \sum_{r=1}^{|D_\ell|-1} \chi_\ell(-r) e^{\frac{2\pi i r}{|D_\ell|}} \\
    &= -G(1,\chi_\ell),
\end{align*}
which implies that $G(1,\chi_\ell)= \pm i \sqrt{|D_\ell|}$.
All together, this shows 
\begin{align*}
   \frac{\sqrt{|D_\ell|}L_\ell(2m+1)}{(2\pi)^{2m+1}} =  \pm \frac{(-1)^{m}}{2|D_\ell|^{2m} (2m)! } L(-2m,\chi_\ell)  \in \Q.
\end{align*}
